On Low Rank Fusion Rings

We present a method to generate all fusion rings of a specific rank and multiplicity. This method was used to generate exhaustive lists of fusion rings up to order 9 for several multiplicities. We introduce a class of non-commutative fusion rings based on a group with transitive action on a set. This generalizes the Tambara-Yamagami (TY) and Haagerup- Izumi (HI) fusion rings. We give an example of such a ring which is categorifiable and is not of TY or HI type. The structure of non-commutative fusion rings with a subgroup is reviewed, and the one-and two-particle extensions of groups are classified. A website containing data on fusion rings is introduced, and an overview of a Wolfram Language package for working with these rings is given.

==> MultFreeFusionRings.tex <==
\begin{longtable}{lllllllll}
\hline
Name & Common name & $r$ & $n$ & $N$ & $𝒟_{PF}$ & $𝒟_{PF}^2$ & Abelian & Group \\
\hline
$\text{FR}_{1}^{1,0}$ & $\text{Trivial}$ & 1 & 0 & 1 & 1.0000 & 1.000 & True & True \\
$\text{FR}_{1}^{2,0}$ & $\mathbb{Z}_2$ & 2 & 0 & 4 & 1.4142 & 2.000 & True & True \\
$\text{FR}_{2}^{2,0}$ & $\text{Fib}$ & 2 & 0 & 5 & 1.9021 & 3.618 & True & False \\
$\text{FR}_{1}^{3,0}$ & $\text{Ising}$ & 3 & 0 & 10 & 2.000 & 4.000 & True & False \\
$\text{FR}_{2}^{3,0}$ & $\left.\text{Rep(}D_3\right)$ & 3 & 0 & 11 & 2.449 & 6.000 & True & False \\
$\text{FR}_{3}^{3,0}$ & $\text{PSU}(2)_5$ & 3 & 0 & 14 & 3.049 & 9.296 & True & False \\
$\text{FR}_{1}^{3,2}$ & $\mathbb{Z}_3$ & 3 & 2 & 9 & 1.7321 & 3.000 & True & True \\
$\text{FR}_{1}^{4,0}$ & $\mathbb{Z}_2\times \mathbb{Z}_2$ & 4 & 0 & 16 & 2.000 & 4.000 & True & True \\
$\text{FR}_{2}^{4,0}$ & $\text{SU(2})_3$ & 4 & 0 & 20 & 2.690 & 7.236 & True & False \\
$\text{FR}_{3}^{4,0}$ & $\left.\text{Rep(}D_5\right)$ & 4 & 0 & 22 & 3.162 & 10.00 & True & False \\
$\text{FR}_{4}^{4,0}$ & $\text{PSU(2})_6$ & 4 & 0 & 24 & 3.696 & 13.66 & True & False \\
$\text{FR}_{5}^{4,0}$ & $\text{Fib$\times $Fib}$ & 4 & 0 & 25 & 3.618 & 13.09 & True & False \\
$\text{FR}_{6}^{4,0}$ & $\text{PSU(2})_7$ & 4 & 0 & 30 & 4.386 & 19.23 & True & False \\
$\text{FR}_{1}^{4,2}$ & $\mathbb{Z}_4$ & 4 & 2 & 16 & 2.000 & 4.000 & True & True \\
$\text{FR}_{2}^{4,2}$ & $\text{Potts}$ & 4 & 2 & 18 & 2.449 & 6.000 & True & False \\
$\text{FR}_{3}^{4,2}$ & $\left.\text{Fib(}\mathbb{Z}_3\right)$ & 4 & 2 & 19 & 2.881 & 8.303 & True & False \\
$\text{FR}_{4}^{4,2}$ & $\text{Pseudo PSU(2})_6$ & 4 & 2 & 24 & 3.696 & 13.66 & True & False \\
$\text{FR}_{1}^{5,0}$ & $\left.\text{Rep(}D_4\right)$ & 5 & 0 & 28 & 2.828 & 8.000 & True & False \\
$\text{FR}_{2}^{5,0}$ & $\left.\text{Fib(}\mathbb{Z}_2\times \mathbb{Z}_2\right)$ & 5 & 0 & 29 & 3.250 & 10.56 & True & False \\
$\text{FR}_{3}^{5,0}$ & $\text{SU(2})_4$ & 5 & 0 & 35 & 3.464 & 12.00 & True & False \\
$\text{FR}_{4}^{5,0}$ & $\left.\text{Rep(}D_7\right)$ & 5 & 0 & 37 & 3.742 & 14.00 & True & False \\
$\text{FR}_{5}^{5,0}$ &   & 5 & 0 & 39 & 4.075 & 16.61 & True & False \\
$\text{FR}_{6}^{5,0}$ & $\left.\text{Rep(}S_4\right)$ & 5 & 0 & 43 & 4.899 & 24.00 & True & False \\
$\text{FR}_{7}^{5,0}$ & $\text{PSU(2})_8$ & 5 & 0 & 45 & 5.117 & 26.18 & True & False \\
$\text{FR}_{8}^{5,0}$ &   & 5 & 0 & 48 & 5.576 & 31.09 & True & False \\
$\text{FR}_{9}^{5,0}$ &   & 5 & 0 & 53 & 5.490 & 30.14 & True & False \\
$\text{FR}_{10}^{5,0}$ & $\text{PSU(2})_9$ & 5 & 0 & 55 & 5.886 & 34.65 & True & False \\
$\text{FR}_{1}^{5,2}$ & $\left.\text{TY(}\mathbb{Z}_4\right)$ & 5 & 2 & 28 & 2.828 & 8.000 & True & False \\
$\text{FR}_{2}^{5,2}$ & $\left.\text{Fib(}\mathbb{Z}_4\right)$ & 5 & 2 & 29 & 3.250 & 10.56 & True & False \\
$\text{FR}_{3}^{5,2}$ & $\text{Pseudo SU(2})_4$ & 5 & 2 & 35 & 3.464 & 12.00 & True & False \\
$\text{FR}_{4}^{5,2}$ & $\left.\text{Pseudo Rep(}S_4\right)$ & 5 & 2 & 43 & 4.899 & 24.00 & True & False \\
$\text{FR}_{5}^{5,2}$ &   & 5 & 2 & 48 & 5.576 & 31.09 & True & False \\
$\text{FR}_{1}^{5,4}$ & $\mathbb{Z}_5$ & 5 & 4 & 25 & 2.236 & 5.000 & True & True \\
$\text{FR}_{1}^{6,0}$ & $\mathbb{Z}_2\text{$\times $Ising}$ & 6 & 0 & 40 & 2.828 & 8.000 & True & False \\
$\text{FR}_{2}^{6,0}$ & $\left.\mathbb{Z}_2\text{$\times $Rep(}D_3\right)$ & 6 & 0 & 44 & 3.464 & 12.00 & True & False \\
$\text{FR}_{3}^{6,0}$ &   & 6 & 0 & 48 & 4.351 & 18.93 & True & False \\
$\text{FR}_{4}^{6,0}$ & $\text{TriCritIsing}$ & 6 & 0 & 50 & 3.804 & 14.47 & True & False \\
$\text{FR}_{5}^{6,0}$ & $\left.\text{Fib$\times $Rep(}D_3\right)$ & 6 & 0 & 55 & 4.659 & 21.71 & True & False \\
$\text{FR}_{6}^{6,0}$ & $\text{SU(2})_5$ & 6 & 0 & 56 & 4.312 & 18.59 & True & False \\
$\text{FR}_{7}^{6,0}$ &   & 6 & 0 & 56 & 4.243 & 18.00 & True & False \\
$\text{FR}_{8}^{6,0}$ &   & 6 & 0 & 56 & 4.243 & 18.00 & True & False \\
$\text{FR}_{9}^{6,0}$ &   & 6 & 0 & 58 & 4.472 & 20.00 & True & False \\
$\text{FR}_{10}^{6,0}$ &   & 6 & 0 & 62 & 5.058 & 25.58 & True & False \\
$\text{FR}_{11}^{6,0}$ &   & 6 & 0 & 65 & 5.328 & 28.39 & True & False \\
$\text{FR}_{12}^{6,0}$ &   & 6 & 0 & 65 & 5.328 & 28.39 & True & False \\
$\text{FR}_{13}^{6,0}$ &   & 6 & 0 & 66 & 5.814 & 33.80 & True & False \\
$\text{FR}_{14}^{6,0}$ & $\left.\text{Fib$\times $ExtRep(}D_3\right)$ & 6 & 0 & 70 & 5.799 & 33.63 & True & False \\
$\text{FR}_{15}^{6,0}$ &   & 6 & 0 & 72 & 6.065 & 36.78 & True & False \\
$\text{FR}_{16}^{6,0}$ & $\text{PSU}(2)_{10}$ & 6 & 0 & 76 & 6.692 & 44.78 & True & False \\
$\text{FR}_{17}^{6,0}$ &   & 6 & 0 & 83 & 7.426 & 55.14 & True & False \\
$\text{FR}_{18}^{6,0}$ & $\text{PSU}(2)_{11}$ & 6 & 0 & 91 & 7.533 & 56.75 & True & False \\
$\text{FR}_{19}^{6,0}$ &   & 6 & 0 & 101 & 7.947 & 63.15 & True & False \\
$\text{FR}_{20}^{6,0}$ &   & 6 & 0 & 101 & 7.947 & 63.15 & True & False \\
$\text{FR}_{1}^{6,2}$ & $D_3$ & 6 & 2 & 36 & 2.449 & 6.000 & False & True \\
$\text{FR}_{2}^{6,2}$ &   & 6 & 2 & 40 & 2.828 & 8.000 & True & False \\
$\text{FR}_{3}^{6,2}$ &   & 6 & 2 & 40 & 2.828 & 8.000 & True & False \\
$\text{FR}_{4}^{6,2}$ & $\left.\text{Rep(}\text{Dic}_{12}\right)$ & 6 & 2 & 44 & 3.464 & 12.00 & True & False \\
$\text{FR}_{5}^{6,2}$ &   & 6 & 2 & 48 & 4.351 & 18.93 & True & False \\
$\text{FR}_{6}^{6,2}$ &   & 6 & 2 & 48 & 4.351 & 18.93 & True & False \\
$\text{FR}_{7}^{6,2}$ & $\text{Pseudo SO(5})_2$ & 6 & 2 & 58 & 4.472 & 20.00 & True & False \\
$\text{FR}_{8}^{6,2}$ & $\left.\text{HI(}\mathbb{Z}_3\right)$ & 6 & 2 & 63 & 5.977 & 35.72 & False & False \\
$\text{FR}_{9}^{6,2}$ &   & 6 & 2 & 66 & 5.814 & 33.80 & True & False \\
$\text{FR}_{10}^{6,2}$ &   & 6 & 2 & 72 & 6.065 & 36.78 & True & False \\
$\text{FR}_{11}^{6,2}$ &   & 6 & 2 & 83 & 7.426 & 55.14 & True & False \\
$\text{FR}_{1}^{6,4}$ & $\mathbb{Z}_6$ & 6 & 4 & 36 & 2.449 & 6.000 & True & True \\
$\text{FR}_{2}^{6,4}$ & $\text{MR}_6$ & 6 & 4 & 40 & 2.828 & 8.000 & True & False \\
$\text{FR}_{3}^{6,4}$ & $\left.\text{TY(}\mathbb{Z}_5\right)$ & 6 & 4 & 40 & 3.162 & 10.00 & True & False \\
$\text{FR}_{4}^{6,4}$ &   & 6 & 4 & 41 & 3.576 & 12.79 & True & False \\
$\text{FR}_{5}^{6,4}$ & $\text{Fib$\times $}\mathbb{Z}_3$ & 6 & 4 & 45 & 3.295 & 10.85 & True & False \\
$\text{FR}_{6}^{6,4}$ &   & 6 & 4 & 48 & 4.351 & 18.93 & True & False \\
$\text{FR}_{7}^{6,4}$ &   & 6 & 4 & 54 & 4.526 & 20.49 & True & False \\
$\text{FR}_{8}^{6,4}$ &   & 6 & 4 & 63 & 5.977 & 35.72 & True & False \\
$\text{FR}_{1}^{7,0}$ &   & 7 & 0 & 64 & 4.000 & 16.00 & True & False \\
$\text{FR}_{2}^{7,0}$ &   & 7 & 0 & 68 & 4.596 & 21.12 & True & False \\
$\text{FR}_{3}^{7,0}$ &   & 7 & 0 & 71 & 5.211 & 27.15 & True & False \\
$\text{FR}_{4}^{7,0}$ &   & 7 & 0 & 72 & 5.380 & 28.94 & True & False \\
$\text{FR}_{5}^{7,0}$ &   & 7 & 0 & 74 & 5.428 & 29.46 & True & False \\
$\text{FR}_{6}^{7,0}$ &   & 7 & 0 & 79 & 4.690 & 22.00 & True & False \\
$\text{FR}_{7}^{7,0}$ & $\text{SU}(2)_6$ & 7 & 0 & 84 & 5.226 & 27.31 & True & False \\
$\text{FR}_{8}^{7,0}$ &   & 7 & 0 & 85 & 5.292 & 28.00 & True & False \\
$\text{FR}_{9}^{7,0}$ &   & 7 & 0 & 89 & 5.864 & 34.39 & True & False \\
$\text{FR}_{10}^{7,0}$ &   & 7 & 0 & 93 & 6.581 & 43.31 & True & False \\
$\text{FR}_{11}^{7,0}$ &   & 7 & 0 & 94 & 6.080 & 36.97 & True & False \\
$\text{FR}_{12}^{7,0}$ &   & 7 & 0 & 99 & 6.481 & 42.00 & True & False \\
$\text{FR}_{13}^{7,0}$ &   & 7 & 0 & 103 & 7.275 & 52.93 & True & False \\
$\text{FR}_{14}^{7,0}$ & $\text{PSU}(2)_{12}$ & 7 & 0 & 119 & 8.407 & 70.68 & True & False \\
$\text{FR}_{15}^{7,0}$ &   & 7 & 0 & 129 & 9.037 & 81.67 & True & False \\
$\text{FR}_{16}^{7,0}$ &   & 7 & 0 & 131 & 9.332 & 87.09 & True & False \\
$\text{FR}_{17}^{7,0}$ & $\text{PSU}(2)_{13}$ & 7 & 0 & 140 & 9.314 & 86.75 & True & False \\
$\text{FR}_{18}^{7,0}$ &   & 7 & 0 & 175 & 10.869 & 118.1 & True & False \\
$\text{FR}_{1}^{7,2}$ &   & 7 & 2 & 54 & 3.464 & 12.00 & False & False \\
$\text{FR}_{2}^{7,2}$ &   & 7 & 2 & 55 & 3.873 & 15.00 & False & False \\
$\text{FR}_{3}^{7,2}$ &   & 7 & 2 & 64 & 4.000 & 16.00 & True & False \\
$\text{FR}_{4}^{7,2}$ &   & 7 & 2 & 64 & 4.000 & 16.00 & True & False \\
$\text{FR}_{5}^{7,2}$ &   & 7 & 2 & 68 & 4.596 & 21.12 & True & False \\
$\text{FR}_{6}^{7,2}$ &   & 7 & 2 & 71 & 5.211 & 27.15 & True & False \\
$\text{FR}_{7}^{7,2}$ &   & 7 & 2 & 71 & 5.211 & 27.15 & True & False \\
$\text{FR}_{8}^{7,2}$ &   & 7 & 2 & 72 & 5.380 & 28.94 & True & False \\
$\text{FR}_{9}^{7,2}$ &   & 7 & 2 & 72 & 5.380 & 28.94 & True & False \\
$\text{FR}_{10}^{7,2}$ &   & 7 & 2 & 74 & 5.428 & 29.46 & True & False \\
$\text{FR}_{11}^{7,2}$ &   & 7 & 2 & 84 & 5.226 & 27.31 & True & False \\
$\text{FR}_{12}^{7,2}$ &   & 7 & 2 & 85 & 5.292 & 28.00 & True & False \\
$\text{FR}_{13}^{7,2}$ &   & 7 & 2 & 93 & 6.581 & 43.31 & True & False \\
$\text{FR}_{14}^{7,2}$ &   & 7 & 2 & 103 & 7.275 & 52.93 & True & False \\
$\text{FR}_{15}^{7,2}$ &   & 7 & 2 & 108 & 8.427 & 71.01 & False & False \\
$\text{FR}_{16}^{7,2}$ &   & 7 & 2 & 129 & 9.037 & 81.67 & True & False \\
$\text{FR}_{17}^{7,2}$ &   & 7 & 2 & 131 & 9.332 & 87.09 & True & False \\
$\text{FR}_{1}^{7,4}$ & $\left.\text{TY(}\mathbb{Z}_2\times \mathbb{Z}_3\right)$ & 7 & 4 & 54 & 3.464 & 12.00 & True & False \\
$\text{FR}_{2}^{7,4}$ &   & 7 & 4 & 55 & 3.873 & 15.00 & True & False \\
$\text{FR}_{3}^{7,4}$ &   & 7 & 4 & 64 & 4.000 & 16.00 & True & False \\
$\text{FR}_{4}^{7,4}$ &   & 7 & 4 & 71 & 5.211 & 27.15 & True & False \\
$\text{FR}_{5}^{7,4}$ &   & 7 & 4 & 72 & 5.380 & 28.94 & True & False \\
$\text{FR}_{6}^{7,4}$ &   & 7 & 4 & 100 & 7.565 & 57.24 & True & False \\
$\text{FR}_{7}^{7,4}$ &   & 7 & 4 & 108 & 8.427 & 71.01 & True & False \\
$\text{FR}_{1}^{7,6}$ & $\mathbb{Z}_7$ & 7 & 6 & 49 & 2.646 & 7.000 & True & True \\
$\text{FR}_{1}^{8,0}$ & $\mathbb{Z}_2\times \mathbb{Z}_2\times \mathbb{Z}_2$ & 8 & 0 & 64 & 2.828 & 8.000 & True & True \\
$\text{FR}_{2}^{8,0}$ & $\text{Fib$\times $}\mathbb{Z}_2\times \mathbb{Z}_2$ & 8 & 0 & 80 & 3.804 & 14.47 & True & False \\
$\text{FR}_{3}^{8,0}$ & $\text{Rep(}D_5\text{)$\times $}\mathbb{Z}_2$ & 8 & 0 & 88 & 4.472 & 20.00 & True & False \\
$\text{FR}_{4}^{8,0}$ &   & 8 & 0 & 92 & 4.899 & 24.00 & True & False \\
$\text{FR}_{5}^{8,0}$ & $\text{PSU}(2)_6\times \mathbb{Z}_2$ & 8 & 0 & 96 & 5.226 & 27.31 & True & False \\
$\text{FR}_{6}^{8,0}$ &   & 8 & 0 & 96 & 5.477 & 30.00 & True & False \\
$\text{FR}_{7}^{8,0}$ & $\text{Fib$\times $Fib$\times $}\mathbb{Z}_2$ & 8 & 0 & 100 & 5.117 & 26.18 & True & False \\
$\text{FR}_{8}^{8,0}$ &   & 8 & 0 & 100 & 6.212 & 38.58 & True & False \\
$\text{FR}_{9}^{8,0}$ &   & 8 & 0 & 106 & 5.099 & 26.00 & True & False \\
$\text{FR}_{10}^{8,0}$ &   & 8 & 0 & 108 & 6.516 & 42.46 & True & False \\
$\text{FR}_{11}^{8,0}$ & $\left.\text{Fib$\times $}\text{Rep}(D_5\right)$ & 8 & 0 & 110 & 6.015 & 36.18 & True & False \\
$\text{FR}_{12}^{8,0}$ &   & 8 & 0 & 112 & 6.902 & 47.63 & True & False \\
$\text{FR}_{13}^{8,0}$ &   & 8 & 0 & 116 & 6.000 & 36.00 & True & False \\
$\text{FR}_{14}^{8,0}$ &   & 8 & 0 & 116 & 6.000 & 36.00 & True & False \\
$\text{FR}_{15}^{8,0}$ & $\text{SU}(2)_7$ & 8 & 0 & 120 & 6.202 & 38.47 & True & False \\
$\text{FR}_{16}^{8,0}$ & $\text{Fib$\times $}\text{PSU}(2)_6$ & 8 & 0 & 120 & 7.029 & 49.41 & True & False \\
$\text{FR}_{17}^{8,0}$ &   & 8 & 0 & 120 & 6.564 & 43.08 & True & False \\
$\text{FR}_{18}^{8,0}$ &   & 8 & 0 & 120 & 6.564 & 43.08 & True & False \\
$\text{FR}_{19}^{8,0}$ &   & 8 & 0 & 124 & 8.286 & 68.66 & True & False \\
$\text{FR}_{20}^{8,0}$ &   & 8 & 0 & 124 & 7.256 & 52.65 & True & False \\
$\text{FR}_{21}^{8,0}$ &   & 8 & 0 & 124 & 7.256 & 52.65 & True & False \\
$\text{FR}_{22}^{8,0}$ & $\text{Fib$\times $Fib$\times $Fib}$ & 8 & 0 & 125 & 6.882 & 47.36 & True & False \\
$\text{FR}_{23}^{8,0}$ & $\left.\text{HI}(\mathbb{Z}_2\times \mathbb{Z}_2\right)$ & 8 & 0 & 128 & 8.705 & 75.78 & True & False \\
$\text{FR}_{24}^{8,0}$ &   & 8 & 0 & 130 & 6.933 & 48.07 & True & False \\
$\text{FR}_{25}^{8,0}$ &   & 8 & 0 & 142 & 7.623 & 58.12 & True & False \\
$\text{FR}_{26}^{8,0}$ &   & 8 & 0 & 142 & 7.623 & 58.12 & True & False \\
$\text{FR}_{27}^{8,0}$ & $\text{Fib$\times $}\text{PSU}(2)_7$ & 8 & 0 & 150 & 8.342 & 69.59 & True & False \\
$\text{FR}_{28}^{8,0}$ &   & 8 & 0 & 151 & 8.485 & 72.00 & True & False \\
$\text{FR}_{29}^{8,0}$ &   & 8 & 0 & 151 & 8.485 & 72.00 & True & False \\
$\text{FR}_{30}^{8,0}$ &   & 8 & 0 & 160 & 8.841 & 78.16 & True & False \\
$\text{FR}_{31}^{8,0}$ & $\text{PSU}(2)_{14}$ & 8 & 0 & 176 & 10.252 & 105.1 & True & False \\
$\text{FR}_{32}^{8,0}$ &   & 8 & 0 & 187 & 11.248 & 126.5 & True & False \\
$\text{FR}_{33}^{8,0}$ &   & 8 & 0 & 187 & 11.248 & 126.5 & True & False \\
$\text{FR}_{34}^{8,0}$ &   & 8 & 0 & 194 & 11.321 & 128.2 & True & False \\
$\text{FR}_{35}^{8,0}$ &   & 8 & 0 & 196 & 11.071 & 122.6 & True & False \\
$\text{FR}_{36}^{8,0}$ & $\text{PSU}(2)_{15}$ & 8 & 0 & 204 & 11.219 & 125.9 & True & False \\
$\text{FR}_{37}^{8,0}$ &   & 8 & 0 & 208 & 11.857 & 140.6 & True & False \\
$\text{FR}_{38}^{8,0}$ &   & 8 & 0 & 281 & 14.182 & 201.1 & True & False \\
$\text{FR}_{1}^{8,2}$ & $D_4$ & 8 & 2 & 64 & 2.828 & 8.000 & False & True \\
$\text{FR}_{2}^{8,2}$ &   & 8 & 2 & 72 & 3.464 & 12.00 & False & False \\
$\text{FR}_{3}^{8,2}$ &   & 8 & 2 & 76 & 4.075 & 16.61 & False & False \\
$\text{FR}_{4}^{8,2}$ &   & 8 & 2 & 80 & 4.899 & 24.00 & False & False \\
$\text{FR}_{5}^{8,2}$ &   & 8 & 2 & 88 & 4.472 & 20.00 & True & False \\
$\text{FR}_{6}^{8,2}$ &   & 8 & 2 & 88 & 4.472 & 20.00 & False & False \\
$\text{FR}_{7}^{8,2}$ &   & 8 & 2 & 92 & 4.899 & 24.00 & True & False \\
$\text{FR}_{8}^{8,2}$ &   & 8 & 2 & 96 & 5.226 & 27.31 & False & False \\
$\text{FR}_{9}^{8,2}$ &   & 8 & 2 & 96 & 5.226 & 27.31 & False & False \\
$\text{FR}_{10}^{8,2}$ &   & 8 & 2 & 96 & 5.226 & 27.31 & False & False \\
$\text{FR}_{11}^{8,2}$ &   & 8 & 2 & 100 & 5.117 & 26.18 & False & False \\
$\text{FR}_{12}^{8,2}$ &   & 8 & 2 & 100 & 6.212 & 38.58 & True & False \\
$\text{FR}_{13}^{8,2}$ &   & 8 & 2 & 108 & 6.516 & 42.46 & True & False \\
$\text{FR}_{14}^{8,2}$ &   & 8 & 2 & 116 & 6.000 & 36.00 & True & False \\
$\text{FR}_{15}^{8,2}$ &   & 8 & 2 & 116 & 6.000 & 36.00 & True & False \\
$\text{FR}_{16}^{8,2}$ &   & 8 & 2 & 124 & 8.286 & 68.66 & True & False \\
$\text{FR}_{17}^{8,2}$ &   & 8 & 2 & 124 & 7.256 & 52.65 & True & False \\
$\text{FR}_{18}^{8,2}$ &   & 8 & 2 & 124 & 7.256 & 52.65 & True & False \\
$\text{FR}_{19}^{8,2}$ & $\left.\text{HI}(\mathbb{Z}_4\right)$ & 8 & 2 & 128 & 8.705 & 75.78 & False & False \\
$\text{FR}_{20}^{8,2}$ &   & 8 & 2 & 128 & 8.705 & 75.78 & False & False \\
$\text{FR}_{21}^{8,2}$ &   & 8 & 2 & 130 & 6.933 & 48.07 & True & False \\
$\text{FR}_{22}^{8,2}$ &   & 8 & 2 & 142 & 7.623 & 58.12 & True & False \\
$\text{FR}_{23}^{8,2}$ &   & 8 & 2 & 142 & 7.623 & 58.12 & True & False \\
$\text{FR}_{24}^{8,2}$ &   & 8 & 2 & 151 & 8.485 & 72.00 & True & False \\
$\text{FR}_{25}^{8,2}$ &   & 8 & 2 & 151 & 8.485 & 72.00 & True & False \\
$\text{FR}_{26}^{8,2}$ &   & 8 & 2 & 187 & 11.248 & 126.5 & True & False \\
$\text{FR}_{27}^{8,2}$ &   & 8 & 2 & 187 & 11.248 & 126.5 & True & False \\
$\text{FR}_{28}^{8,2}$ &   & 8 & 2 & 194 & 11.321 & 128.2 & True & False \\
$\text{FR}_{29}^{8,2}$ &   & 8 & 2 & 196 & 11.071 & 122.6 & False & False \\
$\text{FR}_{30}^{8,2}$ &   & 8 & 2 & 208 & 11.857 & 140.6 & False & False \\
$\text{FR}_{1}^{8,4}$ & $\mathbb{Z}_2\times \mathbb{Z}_4$ & 8 & 4 & 64 & 2.828 & 8.000 & True & True \\
$\text{FR}_{2}^{8,4}$ &   & 8 & 4 & 72 & 3.464 & 12.00 & False & False \\
$\text{FR}_{3}^{8,4}$ & $\mathbb{Z}_2\text{$\times $Potts}$ & 8 & 4 & 72 & 3.464 & 12.00 & True & False \\
$\text{FR}_{4}^{8,4}$ & $\left.\mathbb{Z}_2\text{$\times $Fib(}\mathbb{Z}_3\right)$ & 8 & 4 & 76 & 4.075 & 16.61 & True & False \\
$\text{FR}_{5}^{8,4}$ &   & 8 & 4 & 80 & 4.899 & 24.00 & False & False \\
$\text{FR}_{6}^{8,4}$ &   & 8 & 4 & 80 & 4.899 & 24.00 & True & False \\
$\text{FR}_{7}^{8,4}$ & $\text{Fib$\times $}\mathbb{Z}_4$ & 8 & 4 & 80 & 3.804 & 14.47 & True & False \\
$\text{FR}_{8}^{8,4}$ &   & 8 & 4 & 88 & 4.472 & 20.00 & False & False \\
$\text{FR}_{9}^{8,4}$ & $\text{Fib$\times $Potts}$ & 8 & 4 & 90 & 4.659 & 21.71 & True & False \\
$\text{FR}_{10}^{8,4}$ & $\left.\text{Fib$\times $Fib(}\mathbb{Z}_3\right)$ & 8 & 4 & 95 & 5.481 & 30.04 & True & False \\
$\text{FR}_{11}^{8,4}$ &   & 8 & 4 & 96 & 5.226 & 27.31 & True & False \\
$\text{FR}_{12}^{8,4}$ &   & 8 & 4 & 96 & 5.226 & 27.31 & True & False \\
$\text{FR}_{13}^{8,4}$ & $\left.\mathbb{Z}_2\text{$\times $(Peudo }\text{PSU}(2)_6\right)$ & 8 & 4 & 96 & 5.226 & 27.31 & True & False \\
$\text{FR}_{14}^{8,4}$ &   & 8 & 4 & 112 & 6.902 & 47.63 & True & False \\
$\text{FR}_{15}^{8,4}$ & $\left.\text{Fib$\times $(Peudo }\text{PSU}(2)_6\right)$ & 8 & 4 & 120 & 7.029 & 49.41 & True & False \\
$\text{FR}_{16}^{8,4}$ &   & 8 & 4 & 128 & 8.705 & 75.78 & True & False \\
$\text{FR}_{17}^{8,4}$ &   & 8 & 4 & 128 & 8.705 & 75.78 & True & False \\
$\text{FR}_{18}^{8,4}$ &   & 8 & 4 & 160 & 8.841 & 78.16 & True & False \\
$\text{FR}_{1}^{8,6}$ & $\text{Q}$ & 8 & 6 & 64 & 2.828 & 8.000 & False & True \\
$\text{FR}_{2}^{8,6}$ & $\mathbb{Z}_8$ & 8 & 6 & 64 & 2.828 & 8.000 & True & True \\
$\text{FR}_{3}^{8,6}$ & $\left.\text{TY(}\mathbb{Z}_7\right)$ & 8 & 6 & 70 & 3.742 & 14.00 & True & False \\
$\text{FR}_{4}^{8,6}$ &   & 8 & 6 & 71 & 4.146 & 17.19 & True & False \\
$\text{FR}_{5}^{8,6}$ &   & 8 & 6 & 72 & 3.464 & 12.00 & True & False \\
$\text{FR}_{6}^{8,6}$ &   & 8 & 6 & 80 & 4.899 & 24.00 & True & False \\
$\text{FR}_{7}^{8,6}$ &   & 8 & 6 & 96 & 5.226 & 27.31 & False & False \\
$\text{FR}_{8}^{8,6}$ &   & 8 & 6 & 96 & 5.226 & 27.31 & True & False \\
$\text{FR}_{9}^{8,6}$ &   & 8 & 6 & 128 & 8.705 & 75.78 & False & False \\
$\text{FR}_{10}^{8,6}$ &   & 8 & 6 & 128 & 8.705 & 75.78 & True & False \\
$\text{FR}_{1}^{9,0}$ & $\left.\text{TY(}\mathbb{Z}_2\times \mathbb{Z}_2\times \mathbb{Z}_2\right)$ & 9 & 0 & 88 & 4.000 & 16.00 & True & False \\
$\text{FR}_{2}^{9,0}$ &   & 9 & 0 & 89 & 4.401 & 19.37 & True & False \\
$\text{FR}_{3}^{9,0}$ & $\text{Ising$\times $Ising}$ & 9 & 0 & 100 & 4.000 & 16.00 & True & False \\
$\text{FR}_{4}^{9,0}$ & $\left.\text{Ising$\times $Rep(}D_3\right)$ & 9 & 0 & 110 & 4.899 & 24.00 & True & False \\
$\text{FR}_{5}^{9,0}$ &   & 9 & 0 & 116 & 4.899 & 24.00 & True & False \\
$\text{FR}_{6}^{9,0}$ & $\left.\text{Rep(}D_3\text{)$\times $Rep(}D_3\right)$ & 9 & 0 & 121 & 6.000 & 36.00 & True & False \\
$\text{FR}_{7}^{9,0}$ &   & 9 & 0 & 124 & 5.657 & 32.00 & True & False \\
$\text{FR}_{8}^{9,0}$ &   & 9 & 0 & 128 & 6.225 & 38.74 & True & False \\
$\text{FR}_{9}^{9,0}$ &   & 9 & 0 & 132 & 6.153 & 37.86 & True & False \\
$\text{FR}_{10}^{9,0}$ &   & 9 & 0 & 132 & 6.928 & 48.00 & True & False \\
$\text{FR}_{11}^{9,0}$ &   & 9 & 0 & 132 & 6.153 & 37.86 & True & False \\
$\text{FR}_{12}^{9,0}$ &   & 9 & 0 & 137 & 5.477 & 30.00 & True & False \\
$\text{FR}_{13}^{9,0}$ &   & 9 & 0 & 140 & 7.039 & 49.55 & True & False \\
$\text{FR}_{14}^{9,0}$ & $\text{Ising$\times $}\text{PSU}(2)_5$ & 9 & 0 & 140 & 6.098 & 37.18 & True & False \\
$\text{FR}_{15}^{9,0}$ &   & 9 & 0 & 143 & 7.746 & 60.00 & True & False \\
$\text{FR}_{16}^{9,0}$ &   & 9 & 0 & 148 & 7.664 & 58.74 & True & False \\
$\text{FR}_{17}^{9,0}$ &   & 9 & 0 & 151 & 7.630 & 58.22 & True & False \\
$\text{FR}_{18}^{9,0}$ &   & 9 & 0 & 151 & 7.630 & 58.22 & True & False \\
$\text{FR}_{19}^{9,0}$ &   & 9 & 0 & 151 & 6.633 & 44.00 & True & False \\
$\text{FR}_{20}^{9,0}$ & $\text{Rep(}D_3\text{)$\times $}\text{PSU}(2)_5$ & 9 & 0 & 154 & 7.468 & 55.78 & True & False \\
$\text{FR}_{21}^{9,0}$ &   & 9 & 0 & 155 & 7.191 & 51.71 & True & False \\
$\text{FR}_{22}^{9,0}$ &   & 9 & 0 & 156 & 8.485 & 72.00 & True & False \\
$\text{FR}_{23}^{9,0}$ &   & 9 & 0 & 156 & 8.624 & 74.37 & True & False \\
$\text{FR}_{24}^{9,0}$ &   & 9 & 0 & 159 & 7.865 & 61.86 & True & False \\
$\text{FR}_{25}^{9,0}$ &   & 9 & 0 & 163 & 6.928 & 48.00 & True & False \\
$\text{FR}_{26}^{9,0}$ &   & 9 & 0 & 164 & 9.338 & 87.19 & True & False \\
$\text{FR}_{27}^{9,0}$ & $\text{SU}(2)_8$ & 9 & 0 & 165 & 7.236 & 52.36 & True & False \\
$\text{FR}_{28}^{9,0}$ &   & 9 & 0 & 179 & 7.746 & 60.00 & True & False \\
$\text{FR}_{29}^{9,0}$ &   & 9 & 0 & 185 & 10.408 & 108.3 & True & False \\
$\text{FR}_{30}^{9,0}$ &   & 9 & 0 & 185 & 8.379 & 70.21 & True & False \\
$\text{FR}_{31}^{9,0}$ &   & 9 & 0 & 191 & 9.387 & 88.11 & True & False \\
$\text{FR}_{32}^{9,0}$ &   & 9 & 0 & 195 & 8.784 & 77.17 & True & False \\
$\text{FR}_{33}^{9,0}$ &   & 9 & 0 & 195 & 8.784 & 77.17 & True & False \\
$\text{FR}_{34}^{9,0}$ & $\text{PSU}(2)_5\times \text{PSU}(2)_5$ & 9 & 0 & 196 & 9.296 & 86.41 & True & False \\
$\text{FR}_{35}^{9,0}$ &   & 9 & 0 & 200 & 11.618 & 135.0 & True & False \\
$\text{FR}_{36}^{9,0}$ &   & 9 & 0 & 205 & 9.896 & 97.93 & True & False \\
$\text{FR}_{37}^{9,0}$ &   & 9 & 0 & 211 & 10.023 & 100.5 & True & False \\
$\text{FR}_{38}^{9,0}$ &   & 9 & 0 & 212 & 10.440 & 109.0 & True & False \\
$\text{FR}_{39}^{9,0}$ &   & 9 & 0 & 218 & 10.531 & 110.9 & True & False \\
$\text{FR}_{40}^{9,0}$ &   & 9 & 0 & 227 & 11.428 & 130.6 & True & False \\
$\text{FR}_{41}^{9,0}$ & $\text{PSU}(2)_{16}$ & 9 & 0 & 249 & 12.216 & 149.2 & True & False \\
$\text{FR}_{42}^{9,0}$ &   & 9 & 0 & 256 & 11.708 & 137.1 & True & False \\
$\text{FR}_{43}^{9,0}$ &   & 9 & 0 & 274 & 13.401 & 179.6 & True & False \\
$\text{FR}_{44}^{9,0}$ & $\text{PSU}(2)_{17}$ & 9 & 0 & 285 & 13.241 & 175.3 & True & False \\
$\text{FR}_{45}^{9,0}$ &   & 9 & 0 & 319 & 15.084 & 227.5 & True & False \\
$\text{FR}_{46}^{9,0}$ &   & 9 & 0 & 425 & 17.836 & 318.1 & True & False \\
$\text{FR}_{1}^{9,2}$ &   & 9 & 2 & 88 & 4.000 & 16.00 & False & False \\
$\text{FR}_{2}^{9,2}$ &   & 9 & 2 & 89 & 4.401 & 19.37 & False & False \\
$\text{FR}_{3}^{9,2}$ &   & 9 & 2 & 100 & 4.000 & 16.00 & True & False \\
$\text{FR}_{4}^{9,2}$ &   & 9 & 2 & 108 & 5.447 & 29.67 & False & False \\
$\text{FR}_{5}^{9,2}$ &   & 9 & 2 & 110 & 4.899 & 24.00 & True & False \\
$\text{FR}_{6}^{9,2}$ &   & 9 & 2 & 116 & 4.899 & 24.00 & True & False \\
$\text{FR}_{7}^{9,2}$ &   & 9 & 2 & 116 & 4.899 & 24.00 & False & False \\
$\text{FR}_{8}^{9,2}$ &   & 9 & 2 & 116 & 4.899 & 24.00 & True & False \\
$\text{FR}_{9}^{9,2}$ &   & 9 & 2 & 124 & 5.657 & 32.00 & True & False \\
$\text{FR}_{10}^{9,2}$ &   & 9 & 2 & 124 & 5.657 & 32.00 & True & False \\
$\text{FR}_{11}^{9,2}$ &   & 9 & 2 & 128 & 6.225 & 38.74 & True & False \\
$\text{FR}_{12}^{9,2}$ &   & 9 & 2 & 132 & 6.153 & 37.86 & True & False \\
$\text{FR}_{13}^{9,2}$ &   & 9 & 2 & 132 & 6.153 & 37.86 & True & False \\
$\text{FR}_{14}^{9,2}$ &   & 9 & 2 & 132 & 6.928 & 48.00 & True & False \\
$\text{FR}_{15}^{9,2}$ &   & 9 & 2 & 132 & 6.928 & 48.00 & True & False \\
$\text{FR}_{16}^{9,2}$ &   & 9 & 2 & 132 & 6.153 & 37.86 & True & False \\
$\text{FR}_{17}^{9,2}$ &   & 9 & 2 & 140 & 7.039 & 49.55 & True & False \\
$\text{FR}_{18}^{9,2}$ &   & 9 & 2 & 140 & 7.039 & 49.55 & True & False \\
$\text{FR}_{19}^{9,2}$ &   & 9 & 2 & 143 & 7.746 & 60.00 & True & False \\
$\text{FR}_{20}^{9,2}$ &   & 9 & 2 & 143 & 7.746 & 60.00 & True & False \\
$\text{FR}_{21}^{9,2}$ &   & 9 & 2 & 148 & 7.664 & 58.74 & True & False \\
$\text{FR}_{22}^{9,2}$ &   & 9 & 2 & 148 & 7.664 & 58.74 & False & False \\
$\text{FR}_{23}^{9,2}$ &   & 9 & 2 & 148 & 7.664 & 58.74 & True & False \\
$\text{FR}_{24}^{9,2}$ &   & 9 & 2 & 151 & 7.630 & 58.22 & True & False \\
$\text{FR}_{25}^{9,2}$ &   & 9 & 2 & 151 & 7.630 & 58.22 & True & False \\
$\text{FR}_{26}^{9,2}$ &   & 9 & 2 & 151 & 6.633 & 44.00 & True & False \\
$\text{FR}_{27}^{9,2}$ &   & 9 & 2 & 156 & 8.624 & 74.37 & True & False \\
$\text{FR}_{28}^{9,2}$ &   & 9 & 2 & 156 & 8.624 & 74.37 & True & False \\
$\text{FR}_{29}^{9,2}$ &   & 9 & 2 & 159 & 7.865 & 61.86 & True & False \\
$\text{FR}_{30}^{9,2}$ &   & 9 & 2 & 163 & 6.928 & 48.00 & True & False \\
$\text{FR}_{31}^{9,2}$ &   & 9 & 2 & 164 & 9.338 & 87.19 & True & False \\
$\text{FR}_{32}^{9,2}$ &   & 9 & 2 & 179 & 7.746 & 60.00 & False & False \\
$\text{FR}_{33}^{9,2}$ &   & 9 & 2 & 179 & 7.746 & 60.00 & True & False \\
$\text{FR}_{34}^{9,2}$ &   & 9 & 2 & 195 & 8.784 & 77.17 & True & False \\
$\text{FR}_{35}^{9,2}$ &   & 9 & 2 & 195 & 8.784 & 77.17 & True & False \\
$\text{FR}_{36}^{9,2}$ &   & 9 & 2 & 200 & 11.618 & 135.0 & False & False \\
$\text{FR}_{37}^{9,2}$ &   & 9 & 2 & 200 & 11.618 & 135.0 & False & False \\
$\text{FR}_{38}^{9,2}$ &   & 9 & 2 & 211 & 10.023 & 100.5 & False & False \\
$\text{FR}_{39}^{9,2}$ &   & 9 & 2 & 211 & 10.023 & 100.5 & True & False \\
$\text{FR}_{40}^{9,2}$ &   & 9 & 2 & 227 & 11.428 & 130.6 & True & False \\
$\text{FR}_{41}^{9,2}$ &   & 9 & 2 & 256 & 11.708 & 137.1 & False & False \\
$\text{FR}_{42}^{9,2}$ &   & 9 & 2 & 256 & 11.708 & 137.1 & True & False \\
$\text{FR}_{43}^{9,2}$ &   & 9 & 2 & 274 & 13.401 & 179.6 & True & False \\
$\text{FR}_{44}^{9,2}$ &   & 9 & 2 & 319 & 15.084 & 227.5 & False & False \\
$\text{FR}_{45}^{9,2}$ &   & 9 & 2 & 319 & 15.084 & 227.5 & True & False \\
$\text{FR}_{1}^{9,4}$ & $\left.\text{TY(}\mathbb{Z}_2\times \mathbb{Z}_4\right)$ & 9 & 4 & 88 & 4.000 & 16.00 & True & False \\
$\text{FR}_{2}^{9,4}$ &   & 9 & 4 & 89 & 4.401 & 19.37 & True & False \\
$\text{FR}_{3}^{9,4}$ &   & 9 & 4 & 90 & 3.464 & 12.00 & False & False \\
$\text{FR}_{4}^{9,4}$ &   & 9 & 4 & 100 & 4.000 & 16.00 & False & False \\
$\text{FR}_{5}^{9,4}$ &   & 9 & 4 & 100 & 4.000 & 16.00 & True & False \\
$\text{FR}_{6}^{9,4}$ &   & 9 & 4 & 108 & 5.447 & 29.67 & False & False \\
$\text{FR}_{7}^{9,4}$ &   & 9 & 4 & 108 & 5.447 & 29.67 & True & False \\
$\text{FR}_{8}^{9,4}$ &   & 9 & 4 & 116 & 4.899 & 24.00 & False & False \\
$\text{FR}_{9}^{9,4}$ &   & 9 & 4 & 116 & 4.899 & 24.00 & False & False \\
$\text{FR}_{10}^{9,4}$ &   & 9 & 4 & 116 & 4.899 & 24.00 & True & False \\
$\text{FR}_{11}^{9,4}$ &   & 9 & 4 & 117 & 6.637 & 44.05 & False & False \\
$\text{FR}_{12}^{9,4}$ &   & 9 & 4 & 124 & 5.657 & 32.00 & True & False \\
$\text{FR}_{13}^{9,4}$ &   & 9 & 4 & 132 & 6.153 & 37.86 & True & False \\
$\text{FR}_{14}^{9,4}$ &   & 9 & 4 & 132 & 6.928 & 48.00 & True & False \\
$\text{FR}_{15}^{9,4}$ &   & 9 & 4 & 140 & 7.039 & 49.55 & True & False \\
$\text{FR}_{16}^{9,4}$ &   & 9 & 4 & 143 & 7.746 & 60.00 & True & False \\
$\text{FR}_{17}^{9,4}$ &   & 9 & 4 & 148 & 7.664 & 58.74 & False & False \\
$\text{FR}_{18}^{9,4}$ &   & 9 & 4 & 148 & 7.664 & 58.74 & True & False \\
$\text{FR}_{19}^{9,4}$ &   & 9 & 4 & 156 & 8.624 & 74.37 & True & False \\
$\text{FR}_{20}^{9,4}$ &   & 9 & 4 & 163 & 6.928 & 48.00 & False & False \\
$\text{FR}_{21}^{9,4}$ &   & 9 & 4 & 163 & 6.928 & 48.00 & True & False \\
$\text{FR}_{22}^{9,4}$ &   & 9 & 4 & 164 & 9.338 & 87.19 & False & False \\
$\text{FR}_{23}^{9,4}$ &   & 9 & 4 & 164 & 9.338 & 87.19 & True & False \\
$\text{FR}_{24}^{9,4}$ &   & 9 & 4 & 165 & 7.236 & 52.36 & True & False \\
$\text{FR}_{25}^{9,4}$ &   & 9 & 4 & 185 & 10.408 & 108.3 & True & False \\
$\text{FR}_{26}^{9,4}$ &   & 9 & 4 & 195 & 8.784 & 77.17 & True & False \\
$\text{FR}_{27}^{9,4}$ &   & 9 & 4 & 198 & 9.710 & 94.29 & False & False \\
$\text{FR}_{28}^{9,4}$ &   & 9 & 4 & 200 & 11.618 & 135.0 & True & False \\
$\text{FR}_{29}^{9,4}$ &   & 9 & 4 & 200 & 11.618 & 135.0 & True & False \\
$\text{FR}_{30}^{9,4}$ &   & 9 & 4 & 205 & 9.896 & 97.93 & True & False \\
$\text{FR}_{31}^{9,4}$ &   & 9 & 4 & 227 & 11.428 & 130.6 & False & False \\
$\text{FR}_{32}^{9,4}$ &   & 9 & 4 & 227 & 11.428 & 130.6 & True & False \\
$\text{FR}_{33}^{9,4}$ &   & 9 & 4 & 319 & 15.084 & 227.5 & False & False \\
$\text{FR}_{1}^{9,6}$ &   & 9 & 6 & 88 & 4.000 & 16.00 & False & False \\
$\text{FR}_{2}^{9,6}$ & $\left.\text{TY(}\mathbb{Z}_8\right)$ & 9 & 6 & 88 & 4.000 & 16.00 & True & False \\
$\text{FR}_{3}^{9,6}$ &   & 9 & 6 & 89 & 4.401 & 19.37 & False & False \\
$\text{FR}_{4}^{9,6}$ &   & 9 & 6 & 89 & 4.401 & 19.37 & True & False \\
$\text{FR}_{5}^{9,6}$ & $\text{Ising$\times $}\mathbb{Z}_3$ & 9 & 6 & 90 & 3.464 & 12.00 & True & False \\
$\text{FR}_{6}^{9,6}$ & $\text{Rep(}D_3\text{)$\times $}\mathbb{Z}_3$ & 9 & 6 & 99 & 4.243 & 18.00 & True & False \\
$\text{FR}_{7}^{9,6}$ &   & 9 & 6 & 108 & 5.447 & 29.67 & True & False \\
$\text{FR}_{8}^{9,6}$ &   & 9 & 6 & 108 & 5.328 & 28.39 & True & False \\
$\text{FR}_{9}^{9,6}$ &   & 9 & 6 & 117 & 6.637 & 44.05 & True & False \\
$\text{FR}_{10}^{9,6}$ & $\text{PSU}(2)_5\times \mathbb{Z}_3$ & 9 & 6 & 126 & 5.281 & 27.89 & True & False \\
$\text{FR}_{11}^{9,6}$ &   & 9 & 6 & 162 & 7.428 & 55.17 & True & False \\
$\text{FR}_{12}^{9,6}$ &   & 9 & 6 & 198 & 9.710 & 94.29 & True & False \\
$\text{FR}_{13}^{9,6}$ &   & 9 & 6 & 200 & 11.618 & 135.0 & False & False \\
$\text{FR}_{14}^{9,6}$ &   & 9 & 6 & 200 & 11.618 & 135.0 & True & False \\
$\text{FR}_{15}^{9,6}$ &   & 9 & 6 & 216 & 11.312 & 128.0 & True & False \\
$\text{FR}_{16}^{9,6}$ &   & 9 & 6 & 243 & 12.782 & 163.4 & True & False \\
$\text{FR}_{1}^{9,8}$ & $\mathbb{Z}_9$ & 9 & 8 & 81 & 3.000 & 9.000 & True & True \\
$\text{FR}_{2}^{9,8}$ & $\mathbb{Z}_3\times \mathbb{Z}_3$ & 9 & 8 & 81 & 3.000 & 9.000 & True & True \\
\hline
\end{longtable}


==> detailednoncompergroup.tex <==
\begin{array}{|c|cccc|}
  \hline
  & 6 & 7 & 8 & 9 \\
  \hline
 \mathbb{Z}_2 & 0 & 0 & 3 & 7 \\
 \mathbb{Z}_3 & 1 & 1 & 0 & 1 \\
 \mathbb{Z}_4 & 0 & 0 & 7 & 4 \\
 \mathbb{Z}_2\times \mathbb{Z}_2 & 0 & 0 & 5 & 6 \\
 \mathbb{Z}_6 & 0 & 0 & 0 & 2 \\
 D_3 & 1 & 2 & 5 & 2 \\
 D_4 & 0 & 0 & 1 & 2 \\
 \text{Q} & 0 & 0 & 1 & 2 \\
 \hline
\end{array}

